Enhancing metallicity and basal plane reactivity of 2D materials via self-intercalation

Intercalation (ic) of metal atoms into the van der Waals (vdW) gap of layered materials constitutes a facile strategy to create new materials whose properties can be tuned via the concentration of the intercalated atoms. Here we perform systematic density functional theory calculations to explore various properties of an emergent class of crystalline 2D materials (ic-2D materials) comprising vdW homobilayers with native metal atoms on a sublattice of intercalation sites. From an initial set of 1348 ic-2D materials, generated from 77 vdW homobilayers, we find 95 structures with good thermodynamic stability (formation energy within 200 meV/atom of the convex hull). A significant fraction of the semiconducting host materials are found to undergo an insulator to metal transition upon self-intercalation with only PdS$_2$, PdSe$_2$, and GeS$_2$ maintaining a finite electronic gap. In five cases, self-intercalation introduces magnetism. In general, self-intercalation is found to promote metallicity and enhance the chemical reactivity on the basal plane. Based on the calculated H binding energy we find that self-intercalated SnS$_2$ and Hf$_3$Te$_2$ are promising candidates for hydrogen evolution catalysis. All the stable ic-2D structures and their calculated properties can be explored in the open C2DB database.

==> Tables/table-raw.tex <==
\begin{tabular}{cccccc}
\hline
    Parent ML  &  ic-fraction  &  $\Delta H_{f}$ (eV/atom)  &  $\Delta H_{hull}$ (eV/atom)  &  $E_{gap}$ (eV) & $\mu_{mag}$  \\
\hline
  \ce{Bi2Te3}  &    0.33     &     -0.18     &            45.2            &               0               &              0              \\
  \ce{CrTe2}   &     0.5     &     -0.23     &            3.5             &               0               &            23.88            \\
  \ce{CrTe2}   &      1      &     -0.23     &            16.2            &               0               &            28.74            \\
   \ce{GaTe}   &    0.33     &     -0.32     &            40.3            &               0               &              0              \\
 \ce{HfS2}(T)  &    0.33     &     -1.57     &           -39.2            &               0               &              0              \\
 \ce{HfS2}(T)  &    0.67     &     -1.52     &           -34.2            &               0               &              0              \\
 \ce{HfS2}(T)  &      1      &     -1.4      &            29.8            &               0               &              0              \\
 \ce{HfSe2}(T) &    0.33     &     -1.31     &            4.1             &               0               &              0              \\
 \ce{HfTe2}(T) &    0.33     &     -0.8      &            -2.1            &               0               &              0              \\
 \ce{HfTe2}(T) &    0.67     &     -0.73     &            45.7            &               0               &              0              \\
   \ce{InSe}   &    0.33     &     -0.49     &             24             &               0               &              0              \\
 \ce{NbS2}(H)  &    0.33     &     -1.17     &           -51.6            &               0               &              0              \\
 \ce{NbS2}(T)  &    0.33     &     -1.1      &            23.6            &               0               &              0              \\
 \ce{NbS2}(T)  &    0.67     &     -1.17     &           -12.1            &               0               &              0              \\
 \ce{NbSe2}(H) &    0.33     &     -0.9      &           -10.3            &               0               &              0              \\
 \ce{NbSe2}(H) &    0.67     &     -0.88     &            22.7            &               0               &              0              \\
 \ce{NbSe2}(T) &    0.33     &     -0.85     &            41.8            &               0               &              0              \\
   \ce{PdS2}   &    0.25     &     -0.27     &            30.5            &             0.75              &              0              \\
  \ce{PdSe2}   &    0.25     &     -0.28     &            13.1            &             0.79              &              0              \\
  \ce{PdSe2}   &     0.5     &     -0.27     &            32.8            &             0.71              &              0              \\
 \ce{SnS2}(T)  &    0.33     &     -0.38     &            35.5            &               0               &              0              \\
 \ce{SnSe2}(T) &    0.33     &     -0.36     &            9.8             &               0               &              0              \\
 \ce{SnSe2}(T) &    0.67     &     -0.36     &            17.5            &               0               &              0              \\
 \ce{SnSe2}(T) &      1      &     -0.38     &            16.8            &               0               &              0              \\
 \ce{TaS2}(H)  &    0.33     &     -1.13     &           -75.3            &               0               &              0              \\
 \ce{TaS2}(H)  &    0.67     &     -1.09     &           -70.2            &               0               &              0              \\
 \ce{TaS2}(H)  &      1      &     -1.01     &           -17.8            &               0               &              0              \\
 \ce{TaS2}(T)  &    0.33     &     -1.05     &            2.3             &               0               &              0              \\
 \ce{TaS2}(T)  &    0.67     &     -0.99     &            31.4            &               0               &              0              \\
 \ce{TaSe2}(T) &    0.33     &     -0.77     &            34.5            &               0               &              0              \\
 \ce{TiTe2}(T) &    0.33     &     -0.72     &            -6.1            &               0               &              0              \\
 \ce{TiTe2}(T) &    0.67     &     -0.69     &            28.7            &               0               &              0              \\
  \ce{VS2}(H)  &    0.33     &     -0.96     &            -26             &               0               &            1.51             \\
  \ce{VS2}(H)  &    0.67     &     -0.96     &            23.8            &               0               &              0              \\
   \ce{W2N3}   &    0.33     &     -0.32     &            -135            &               0               &              0              \\
   \ce{W2N3}   &    0.67     &     -0.31     &           -121.1           &               0               &              0              \\
   \ce{W2N3}   &      1      &     -0.2      &           -15.6            &               0               &              0              \\
 \ce{ZrSe2}(T) &    0.33     &     -1.38     &           -60.4            &               0               &              0              \\
 \ce{ZrSe2}(T) &    0.67     &     -1.35     &           -65.7            &               0               &              0              \\
 \ce{ZrSe2}(T) &      1      &     -1.3      &           -49.8            &               0               &              0              \\
\hline
\end{tabular}

